Deep Reinforcement Learning Agents are not even close to Human Intelligence

Deep reinforcement learning (RL) agents achieve impressive results in a wide variety of tasks, but they lack zero-shot adaptation capabilities. While most robustness evaluations focus on tasks complexifications, for which human also struggle to maintain performances, no evaluation has been performed on tasks simplifications. To tackle this issue, we introduce HackAtari, a set of task variations of the Arcade Learning Environments. We use it to demonstrate that, contrary to humans, RL agents systematically exhibit huge performance drops on simpler versions of their training tasks, uncovering agents' consistent reliance on shortcuts. Our analysis across multiple algorithms and architectures highlights the persistent gap between RL agents and human behavioral intelligence, underscoring the need for new benchmarks and methodologies that enforce systematic generalization testing beyond static evaluation protocols. Training and testing in the same environment is not enough to obtain agents equipped with human-like intelligence.

==> environment_description/Assault.tex <==
You control a vehicle that can move sideways. A big mother ship circles overhead and continually deploys smaller drones. You must destroy these enemies and dodge their attacks.

==> environment_description/Asteroids.tex <==
This is a well-known arcade game: You control a spaceship in an asteroid field and must break up asteroids by shooting them. Once all asteroids are destroyed, you enter a new level and new asteroids will appear. You will occasionally be attacked by a flying saucer.

==> environment_description/BattleZone.tex <==
You control a tank and must destroy enemy tanks. This game is played in a first-person perspective and creates a 3D illusion. A radar screen shows enemies around you. You start with 5 lives and gain up to 2 extra lives if you reach a sufficient score.

==> environment_description/Berzerk.tex <==
You are stuck in a maze with evil robots. You must destroy them and avoid touching the walls of the maze, as this will kill you. You may be awarded extra lives after scoring a sufficient number of points, depending on the game mode. You may also be chased by an unbeatable enemy, Evil Otto, that you must avoid. Evil Otto does not appear in the default mode.

==> environment_description/Centipede.tex <==
You are an elf and must use your magic wands to fend off spiders, fleas and centipedes. Your goal is to protect mushrooms in an enchanted forest. If you are bitten by a spider, flea or centipede, you will be temporally paralyzed and you will lose a magic wand. The game ends once you have lost all wands. You may receive additional wands after scoring a sufficient number of points.

==> environment_description/CrazyClimber.tex <==
You are a climber trying to reach the top of four buildings, while avoiding obstacles like closing windows and falling objects. When you receive damage (windows closing or being hit by objects) you will fall and lose one life; you have a total of 5 lives before the end games. At the top of each building, there’s a helicopter which you need to catch to get to the next building. The goal is to climb as fast as possible while receiving the least amount of damage.

==> environment_description/Gopher.tex <==
The player controls a shovel-wielding farmer who protects a crop of three carrots from a gopher.

==> environment_description/Hero.tex <==
You need to rescue miners that are stuck in a mine shaft. You have access to various tools: A propeller backpack that allows you to fly wherever you want, sticks of dynamite that can be used to blast through walls, a laser beam to kill vermin, and a raft to float across stretches of lava.You have a limited amount of power. Once you run out, you lose a live.

==> environment_description/IceHockey.tex <==
Your goal is to score as many points as possible in a standard game of Ice Hockey over a 3-minute time period. The ball is usually called “the puck”.There are 32 shot angles ranging from the extreme left to the extreme right. The angles can only aim towards the opponent’s goal.Just as in real hockey, you can pass the puck by shooting it off the sides of the rink. This can be really key when you’re in position to score a goal.

==> environment_description/Krull.tex <==
Your mission is to find and enter the Beast’s Black Fortress, rescue Princess Lyssa, and defeat the Beast. The task is not an easy one, for the location of the Black Fortress changes with each sunrise on Krull.

==> environment_description/Pacman.tex <==
A classic arcade game. Move Pac Man around a maze collecting food and avoiding ghosts- unless you eat a Power Pellet, then you can eat the ghosts too!

==> environment_description/Pitfall.tex <==
You control Pitfall Harry and are tasked with collecting all the treasures in a jungle within 20 minutes. You have three lives. The game is over if you collect all the treasures or if you die or if the time runs out.

==> environment_description/PrivateEye.tex <==
You control the French Private Eye Pierre Touche. Navigate the city streets, parks, secret passages, dead-ends and one-ways in search of the ringleader, Henri Le Fiend and his gang. You also need to find evidence and stolen goods that are scattered about. There are five cases, complete each case before its statute of limitations expires.

==> environment_description/Qbert.tex <==
You are Q*bert. Your goal is to change the color of all the cubes on the pyramid to the pyramid’s ‘destination’ color. To do this, you must hop on each cube on the pyramid one at a time while avoiding nasty creatures that lurk there.

==> environment_description/Riverraid.tex <==
You control a jet that flies over a river: you can move it sideways and fire missiles to destroy enemy objects. Each time an enemy object is destroyed you score points (i.e. rewards). Fly over a fuel depot when you begin to run low, before you lose your jet. You also lose a jet when it collides with the river bank or one of the enemy objects (except fuel depots). The game begins with a squadron of three jets in reserve and you’re given an additional jet (up to 9) for each 10,000 points you score.

==> environment_description/RoadRunner.tex <==
You control the Road Runner(TM) looking for food; you can control the direction to run in and times to jumps. The goal is to outrun Wile E. Coyote(TM) while avoiding the hazards of the desert. The game begins with three lives. You lose a life when the coyote catches you, picks you up in a rocket, or shoots you with a cannon. You also lose a life when a truck hits you, you hit a land mine, you fall off a cliff, or you get hit by a falling rock. You score points (i.e. rewards) by eating seeds along the road, eating steel shot, and destroying the coyote.

==> environment_description/UpNDown.tex <==
Your goal is to steer your baja bugger to collect prizes and eliminate opponents.

==> environment_description/VideoPinball.tex <==
Your goal is to keep the ball in play as long as possible and to score as many points as possible.

==> game_modifs/DoubleDunk.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{3cm} | p{10cm}} \toprule
        \textbf{Modification} & \textbf{Effect} \\ \midrule
        player\_color\_$X$ & Changes the players jersey to the color $X \in$ [white, green, red, yellow, purple, blue]. \\
        enemy\_color\_$X$ & Changes the enemy jersey to the color $X \in$ [white, green, red, yellow, purple, blue]. \\ \bottomrule
    \end{tabular}
    % \label{tab:my_label}
\end{table}

==> game_modifs/NameThisGame.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{3cm} | p{10cm}} \toprule
        \textbf{Modification} & \textbf{Effect} \\ \midrule
        unlimited\_oxygen & Provides the player with an unlimited supply of oxygen. \\
        unlimited\_lives & Player has an unlimited amounts of lives. \\
        double\_wave\_length & Doubles the amount of time it takes to get into the next phase. \\
        quick\_start & Skips the intro. \\ \bottomrule
    \end{tabular}
    % \label{tab:my_label}
\end{table}

==> game_modifs/Seaquest.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{4cm} | p{9cm}} \toprule
        \textbf{Modification} & \textbf{Effect} \\ \midrule
        unlimited\_oxygen & Changes the behavior of the oxygen bar to remain filled\\
        gravity & Enables gravity for the player. \\
        disable\_enemies &  Disables all the enemies.\\
        random\_color\_enemies & The enemies have new random colors each time they go across the screen. \\
        \bottomrule
    \end{tabular}
    % \label{tab:my_label}
\end{table}

==> game_modifs/StarGunner.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{3cm} | p{10cm}} \toprule
        \textbf{Modification} & \textbf{Effect} \\ \midrule
        static\_bomber & Stops the bomber at the top from moving. \\
        static\_flyers & Stops the flying enemies in place. \\
        remove\_mountains & Removes the mountains from the game. \\
        static\_mountains & The mountains stay the same, even if the player moves. \\
        \bottomrule
    \end{tabular}
    % \label{tab:my_label}
\end{table}
